Identifying Possible Rumor Spreaders on Twitter: A Weak Supervised Learning Approach

Online Social Media (OSM) platforms such as Twitter, Facebook are extensively exploited by the users of these platforms for spreading the (mis)information to a large audience effortlessly at a rapid pace. It has been observed that the misinformation can cause panic, fear, and financial loss to society. Thus, it is important to detect and control the misinformation in such platforms before it spreads to the masses. In this work, we focus on rumors, which is one type of misinformation (other types are fake news, hoaxes, etc). One way to control the spread of the rumors is by identifying users who are possibly the rumor spreaders, that is, users who are often involved in spreading the rumors. Due to the lack of availability of rumor spreaders labeled dataset (which is an expensive task), we use publicly available PHEME dataset, which contains rumor and non-rumor tweets information, and then apply a weak supervised learning approach to transform the PHEME dataset into rumor spreaders dataset. We utilize three types of features, that is, user, text, and ego-network features, before applying various supervised learning approaches. In particular, to exploit the inherent network property in this dataset (user-user reply graph), we explore Graph Convolutional Network (GCN), a type of Graph Neural Network (GNN) technique. We compare GCN results with the other approaches: SVM, RF, and LSTM. Extensive experiments performed on the rumor spreaders dataset, where we achieve up to 0.864 value for F1-Score and 0.720 value for AUC-ROC, shows the effectiveness of our methodology for identifying possible rumor spreaders using the GCN technique.

==> Shakshi-Rumor_Spreaders-IJCNN(15 jan 21)/Dataset.tex <==
\section{Dataset Description and Methodology}\label{sec:ds}

In this section, we first discuss the \textbf{PHEME} dataset (Section \ref{sec:OrgDS}). Next, in Section \ref{sec:TranO2S}, we describe how we transform the \textbf{PHEME} tweets dataset into the rumor spreaders dataset. Finally, we explain three different types of features extracted from the dataset, which are provided as input to the machine learning algorithms (Section \ref{sec:FeatExt}).


\subsection{Original Dataset}\label{sec:OrgDS}

This paper utilizes the \textbf{PHEME}\footnote[1]{https://figshare.com/articles/PHEME\textunderscore dataset\textunderscore of\textunderscore rumours\textunderscore and\textunderscore non-rumours/4010619} dataset, which is a collection of \textit{rumor} and \textit{non-rumor} tweets that have been extensively used in previous works \cite{kochkina2018all, zubiaga2018detection}. The dataset comprises five events (or incidents) - \textit{Charlie hebdo}, \textit{German wings crash}, \textit{Ottawa shooting}, \textit{Sydney siege} and \textit{Ferguson}.
For the rest of this work, we refer to them as \textit{Charlie}, \textit{German}, \textit{Ottawa}, \textit{Sydney}, and \textit{Ferguson}, respectively.
%This work utilizes four separate publicly available datasets; Rollcall, Bills identifier, Member of Parliament's (MP's) characteristics \cite{ULeNet} and MP's images which are available on the official website\footnote{https://w1.c1.rada.gov.ua/pls/site2/p\_deputat\_list?skl=9}. For the rest of this work, we refer to them as \textit{Rollcall}, \textit{Identifiers}, \textit{MP's characteristics} and \textit{Facial trait}, respectively.
The dataset contains information about the tweets pertaining to these incidents that have been posted as breaking news during the year 2014 -- 2015.
To be specific, data is provided in the form of five files, where each file is related to five particular incidents. The data in each file is stored in JSON format, having information about the source (or initiator's) tweet and its corresponding information.  Table \ref{Tbl:TweetDesdescp} provides detailed information about various fields. %\st{such as, the user id of the user who wrote that tweet, etc. For each incidents, we extracted 11 fields (see Table \ref{Tbl:TweetDesdescp}). }

\begin{table}[!htbp]
\centering
\caption{Dataset Description}
%\label{data description}
\label{Tbl:TweetDesdescp}
\begin{tabular}{|l|l|l|}
\hline
\textbf{No} & \textbf{Fields}       & \textbf{Description}                               \\ \hline
\textbf{1}  & user id               & unique id of the initiator user                    \\ \hline
\textbf{2}  & tweet                 & tweet posted by initiator                          \\ \hline
\textbf{3}  & \# of followers       & of the initiator                                   \\ \hline
\textbf{4}           & \# of favorites       & of the initiator                                   \\ \hline
\textbf{5}           & verified user         & source user has verified account or not   \\ \hline
\textbf{6}           & reply user id         & unique id of the reply user                        \\ \hline
\textbf{7}           & reply tweet           & tweet posted by reply user                         \\ \hline
\textbf{8}           & \# of reply followers & of the reply user                                  \\ \hline
\textbf{9}           & \# of reply favorites & of the reply user                                  \\ \hline
\textbf{10}          & verified reply user   & reply user has verified account or not             \\ \hline
\textbf{11}          & label                 &  initiator's tweet is rumor or not \\ \hline
\end{tabular}
\end{table}




\begin{comment}
\begin{table}[!htbp]
\centering
\caption{Percentage of rumor and non-rumor tweets for each of the incident in the dataset}
%\label{Descriptive Statistics of data set}
\label{Tbl:DescpStat}
\begin{tabular}{|l|p{14mm}|p{14mm}|}
\hline
\textbf{Incident} & \textbf{\# of rumor tweets} & \textbf{\# of non-rumor tweets} \\ \hline
\textbf{CH}        & 458 (22\%)                 & 1621 (78\%)                   \\ \hline
\textbf{GW}   & 238 (50.7\%)               & 231 (49.3\%)                   \\ \hline
\textbf{OS}      & 470 (52.8\%)               & 420 (47.2\%)                   \\ \hline
\textbf{SS}        & 522 (42.8\%)                 & 699 (57.2\%)                   \\ \hline
\textbf{FG}        & 284 (24.8\%)                 & 859 (75.2\%)                   \\ \hline

\end{tabular}%

\end{table}
\end{comment}

Furthermore, each source tweet has the ground-truth regarding
%with respect to 
whether the tweet is a \textit{rumor} or \textit{non-rumor}. Table \ref{Tbl:DescpStat}, column `\# of Tweets (\%)' provides information about the number of \textit{rumor} and \textit{non-rumor} tweets for each of the incidents
for our analysis. 
\begin{table}[!htbp]
\centering
\caption{Distribution of Tweets and Spreaders for each of the incidents in the dataset}
%\label{Descriptive Statistics of data set}
\label{Tbl:DescpStat}
\begin{tabular}{|l|p{14mm}|p{14mm}|p{14mm}|p{14mm}|}
\hline
\textbf{} & \multicolumn{2}{|c|}{\textbf{\# of Tweets (\%)}} & \multicolumn{2}{|c|}{\textbf{\# of Spreaders (\%)}} \\ \hline
\textbf{Incidents} & \textbf{Rumor} & \textbf{Non-rumor} & \textbf{Rumor} & \textbf{Non-rumor} \\ \hline
\textbf{Charlie}        & 458 (22\%)                 & 1621 (78\%)             &      13879 (74.2\%)                       & 4821  (25.8\%)                \\ \hline
\textbf{German}   & 238 (50.7\%)               & 231 (49.3\%)                 & 1464  (50.3\%)                        & 1442  (49.7\%)                      \\ \hline
\textbf{Ottawa}      & 470 (52.8\%)               & 420 (47.2\%)                   & 3978  (51.1\%)                         & 3794  (48.9\%)                   \\ \hline
\textbf{Sydney}        & 522 (42.8\%)                 & 699 (57.2\%)               & 7545  (61.8\%)                        & 4658  (38.2\%)                   \\ \hline
\textbf{Ferguson}        & 284 (24.8\%)                 & 859 (75.2\%)                & 3792  (35\%)                        & 7001  (65\%)                   \\ \hline

\end{tabular}%
\end{table}

%In Tables \ref{Tbl:DescpStat}-\ref{tbl:datadim}, the term 'CH' represents \textit{Charlie hebdo}, 'GW' represents \textit{German wings crash}, 'OS' represents \textit{Ottawa shooting}, 'SS' represents \textit{Sydney siege}, and 'FG' represents \textit{Ferguson} incident. 


 %\fixme{I am not able to udnerstand --are you tryign to say any responders which are not criticising or questio, you removed them?} \PS{No, It means that people sometimes replies which is out of the context or paste any urls or say rubbish things, etc.}


% RUMOR = 1

\begin{comment}
\begin{table}[!htbp]
\centering
\caption{Percentage of possible rumor spreaders and non-rumor spreaders for each of the incidents in the dataset}
\label{Tbl:DescpStat_suspicioususers}
\begin{tabular}{|l|l|l|}
\hline
\textbf{Incidents} & \textbf{\# of rumor spreaders} & \textbf{\# of non-rumor spreaders} \\ \hline
\textbf{CH}       & 13879 (74.2\%)                       & 4821  (25.8\%)                            \\ \hline
\textbf{GW}  & 1464  (50.3\%)                        & 1442  (49.7\%)                            \\ \hline
\textbf{OS}     & 3978  (51.1\%)                         & 3794  (48.9\%)                         \\ \hline
\textbf{SS}  & 7545  (61.8\%)                        & 4658  (38.2\%)                            \\ \hline
\textbf{FG}  & 3792  (35\%)                        & 7001  (65\%)                            \\ \hline
\end{tabular}%
\end{table}
\end{comment}

\subsection{Transformation of Tweets Dataset into Rumor Spreaders Dataset}\label{sec:TranO2S}


\begin{comment}
    
\begin{figure*}[!htbp]

     \subfloat[Charlie hebdo\label{subfig-1:charlie}]{%
       \includegraphics[width=0.20\textwidth]{Figures/charlie_sentiments.pdf}
     }
       \subfloat[German wings crash\label{subfig-1:german}]{%
       \includegraphics[width=0.20\textwidth]{Figures/german_sentiments.pdf}
     }
     \subfloat[Ottawa shooting\label{subfig-2:ottawa}]{%
       \includegraphics[width=0.20\textwidth]{Figures/ottawa_sentiments.pdf}
     }
      \subfloat[Sydney siege\label{subfig-2:sydney}]{%
       \includegraphics[width=0.20\textwidth]{Figures/sydney_sentiments.pdf}
     } 
      \subfloat[Ferguson\label{subfig-2:ferguson}]{%
       \includegraphics[width=0.20\textwidth]{Figures/ferguson_sentiments.pdf}
     }
     \caption{Sentiments of Reply Tweets with respect to Rumor and Non-Rumor Tweets for all the five incidents}
     \label{fig:Sentiments}
   \end{figure*}
\end{comment}
  
Due to the lack of an annotated dataset of users who are spreading the \textit{rumors} on OSM platforms, we first transform
the \textbf{PHEME} dataset (which carries information pertaining to the initiator's tweets, such as users who replied to the initiator's tweets, the \textit{followers count} of the initiator user, etc.) into the rumor spreaders dataset.
%The dataset carries information pertaining to the initiator's tweets, such as users who replied to the initiator's tweets, the \textit{followers count} of the initiator user, etc.
Table \ref{tbl:datadim}, column `Tweets', shows the original dimensions of the incidents, wherein each cell value represents the total number of initiator's tweets (36189 rows in case of \textit{Charlie}) and the total number of features, including ground-truth labels (11 columns for all the incidents).

\begin{table}[!htbp]
\caption{Dimensions of the \textbf{PHEME} dataset at various levels}
\label{tbl:datadim}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Incidents}  & \textbf{Tweets} & \textbf{Rumor Spreaders} & \textbf{ Adjacency Matrix} \\ \hline
\textbf{Charlie}  & 36189, 11 & 18700, 304 &  18700, 18700 \\ \hline
\textbf{German}  & 4020, 11 & 2906, 304 &  2906, 2906 \\ \hline
\textbf{Ottawa}  & 11394, 11 & 7772, 304 &  7772, 7772 \\ \hline
\textbf{Sydney}  & 22775, 11 & 12203, 304 &  12203, 12203 \\ \hline
\textbf{Ferguson}  & 46064, 11 & 10793, 304 &  10793, 10793 \\ \hline
\end{tabular}
\end{table}


\begin{table*}[!htbp]
\caption{An Example of the Tweets on Ferguson incident}
\label{tbl:desribe}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{No} & \textbf{Initiator Tweet}                                                                                                                                                                      & \textbf{Reply Tweet 1}                                                                                                               & \textbf{Reply Tweet 2}                                                                                                               \\ \hline
1           & \begin{tabular}[c]{@{}l@{}}The mother of the boy killed in \#Ferguson\\ speaking to media about the loss of her son.\\ http://t.co/YlxEDKoebB\end{tabular}                                    & \begin{tabular}[c]{@{}l@{}}@AntonioFrench @b9AcE guess the cops were \\ protecting and serving the community again.\end{tabular}     & \begin{tabular}[c]{@{}l@{}}@AntonioFrench my heart aches \\ for her! This was so wrong!\end{tabular}                                 \\ \hline
2           & \begin{tabular}[c]{@{}l@{}}Police in \#Ferguson once charged a man \\ w/ destruction of property for bleeding \\ on their uniforms after they beat him \\ http://t.co/MRVP76sdUP\end{tabular} & \begin{tabular}[c]{@{}l@{}}@AnonyOps that's not true Dudeee!!\\ please go and read good newspapers. \\ \end{tabular} & \begin{tabular}[c]{@{}l@{}}@RianAlden not at all, but they \\ need to change some things at \\ \#ferguson PD. @AnonyOps\end{tabular} \\ \hline
\end{tabular}%
}
\end{table*}

In order to identify possible \textit{rumor spreaders}, we start by
%tweet-oriented data storage into user-oriented data storage 
placing each user with its corresponding tweets followed by its responders and their respective reply tweets. As part of the data cleaning process, we remove non-alphanumeric characters, URLs, stopwords, punctuations, lowercase all the words and perform additional Natural Language Processing operations as well, for instance, Porter Stemming of the words.
We cover the steps taken for the conversion:

\noindent\textbf{Step 1: Sentiment Analysis of the Reply tweets:}
It is highly likely that a tweet may have attracted multiple responses (or replies). To exemplify, Table \ref{tbl:desribe} shows an example of the two tweets from \textit{Ferguson} incident.
%Table \ref{tbl:desribe} shows an example of the two tweets on \textit{Ferguson} incident. 
The first row corresponds to the \textit{non-rumor} tweet along with its replies (in this Table, we have shown only two replies, but a tweet can have any number of replies), whereas the second row corresponds to the \textit{rumor} tweet. 
It can be seen that the reply tweets possess sentiments with respect to the posted tweet, which can help in identifying the \textit{rumors}, and thus, \textit{rumor spreaders}. For instance,
\textit{non-rumor} tweets are in support of the initiator's tweet, hence, represents a positive sentiment.
%such as, in the form of condolences (in this case) 
Whereas in the case of \textit{rumor} tweets, reply tweets do not show support of the initiator's tweet, indicating negative sentiment. 
%\fixme{break the sentence?} for instance, in the form of verifying \fixme{questioning? may be verifying is better} the veracity of the news or \fixme{add -- rather?} claiming it to be false. \fixme{let us discuss the next line?}\PS{This is applicable to all the reply tweets except noisy ones (that are out of the context of the initiator's tweet and is removed as part of the pre-processing step) present in the dataset.}
This could be a key indication that sentiments of the reply tweets play a key role in identifying whether the tweets posted by the user is \textit{rumor} or not.
%To verify the same, we calculate the sentiments of all the reply tweets for all the incidents.

In this regard, we first try to analyze the sentiments of the reply tweets using \textit{TextBlob API}\footnote[2] {https://textblob.readthedocs.io/en/dev/api\_reference.html}. Figure \ref{fig:Sentiments} displays the sentiments of the reply tweets with respect to \textit{rumor} and \textit{non-rumor} tweets for all five incidents. Specifically, the x-axis represents the positive and negative sentiments with respect to \textit{rumor} and \textit{non-rumor} reply tweets for all the incidents and y-axis corresponds to its percentage.
To capture the same, we consider the reply tweets under the \textit{rumor} category if the initiator's tweet is a \textit{rumor} otherwise \textit{non-rumor}. 
%Y-axis represents the count of reply tweets.
It is clear from Figure \ref{fig:Sentiments} that reply tweets under the \textit{rumor} category have mostly negative sentiments and vice-versa for all the incidents (we have excluded the \# of neutral sentiments, which are very few in number to avoid confusion). 
%Though some of the sentiments under rumor (non-rumor) category is positive (negative) but are very few in number. 
%In addition, it is clear that \textit{rumor} tweets receives more replies as compared to \textit{non-rumor} tweets.
Thus, it can be validated that the sentiments of the reply tweets can be utilized to identify \textit{rumor} tweets, and hence, possible \textit{rumor spreaders}.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=8cm,height=8cm,trim = {0cm 0cm 0cm 0cm}, clip,  keepaspectratio]{Figures/sentiments.PNG}
    \caption{Sentiments of Reply Tweets with respect to Rumor and Non-Rumor Tweets for all the five incidents }\label{fig:Sentiments}
\end{figure}

\begin{comment}
    
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=9cm,height=8cm, keepaspectratio]{Figures/download.png}
    \caption{Sentiments of Reply Tweets with respect to Rumor and Non-Rumor Tweets of Ferguson incident \fixme{I think it is better to show for every dataset?}}\label{fig:Sentiments}
\end{figure}
\end{comment}





\noindent\textbf{Step 2: Labeling Reply tweets Using Weak Supervised Learning Approach:}
In order to identify the possible rumor spreaders, we would like to utilize the stance of reply tweets in our approach. However, no such information is present in the dataset. Thus, in  order  to  label  each  reply  tweet,
%Our main goal is to find whether a particular user is a \textit{possible rumor spreader} or not, and thus, it is important to have the labels for each tweet, whether it is an initiated tweet or reply tweet (See Step 3 for more details). In this context,
%we have the labels for initiated tweets.
%Next, in order to label each reply tweet as a \textit{rumor} or not, 
we apply the \textit{MinHash}\footnote[3] {snaPy API: https://pypi.org/project/snapy/} algorithm in line with \cite{nilizadeh2019think}. The \textit{MinHash} finds the similarities between each pair of the initiator's tweet and the reply tweet.
%for finding similarities between the two.
Specifically, if both these tweets are similar, then we assign the same label to the reply tweet as the initiator's tweet, indicating that the reply tweet is in support of the initiator's tweet. Otherwise, we assign the opposite label to the reply tweet. We considered two tweets to be similar if their similarity score is greater than or equal to 85\% (this threshold is validated manually). This approach of labeling the reply tweets is what we call as weak supervised learning approach due to the fact that we do not have the manual annotation of these tweets.
%detect the stance of the reply tweets. Utilizing the weak supervised learning approach, we apply the \textit{MinHash}\footnote[3] {snaPy API: https://pypi.org/project/snapy/} algorithm in line with \cite{nilizadeh2019think} between each pair of the initiator's tweet and the reply tweet for finding similarities between the two. Specifically, if both the tweets are similar, then we assign the same label to the reply tweet as the initiator's tweet, that is, the reply tweet is in support of the initiator's tweet. Otherwise, we assign the opposite label to the reply tweet. 
%This way, we assign labels to all the reply tweets. 

%In order to identify all the rumor spreaders who are often involved in rumor, we assign a label to each reply tweet.
%To capture the same, we adopted the use of
%the similarity score of the original tweet and its corresponding response. In particular, we calculated \textit{Antonym} and \textit{Jaccard} similarity for each pair of the initiator tweet and its corresponding reply tweet. If there are antonyms or Jaccard similarity between a pair is less than 50 percent, then we assign an opposite label to the reply tweet with respect to the original tweet, signifying that the reply tweet is not in support of the initiator tweet. Otherwise, we assign a similar label to that of the initiator tweet. %\sout{This way}\shakshi{Accordingly,} 
%By using this process, we assign labels to all the reply tweets.


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{comment}
\begin{table}[!htbp]
\caption{Different Data Dimensions \fixme{These Figures and the AUC/ROC Figures need to  be brought earlier.}}
\label{Tbl:DataDim}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{No} &
  \textbf{CH} &
  \textbf{GW} &
  \textbf{OS} &
  \textbf{SS} &
  \textbf{FG} \\ \hline
1 &
  \begin{tabular}[c]{@{}l@{}}(36189, \\ 11)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(4020, \\ 11)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(11394, \\ 11)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(22775,\\  11)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(46064, \\ 11)\end{tabular} \\ \hline
2 &
  \begin{tabular}[c]{@{}l@{}}(18700, \\ 25924)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(2906, \\ 5201)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(7772, \\ 9415)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(12203, \\ 15987)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(10793, \\ 15987)\end{tabular} \\ \hline
3 &
  \begin{tabular}[c]{@{}l@{}}(18700, \\ 3573)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(2906, \\ 766)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(7772, \\ 1656)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(12203, \\ 2660)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(10793,\\  2794)\end{tabular} \\ \hline
4 &
  \begin{tabular}[c]{@{}l@{}}(18700,\\  3574)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(2906, \\ 767)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(7772, \\ 1657)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(12203, \\ 2661)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(10793, \\ 2795)\end{tabular} \\ \hline
5 &
  \begin{tabular}[c]{@{}l@{}}(18700, \\ 18700)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(2906, \\ 2906)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(7772, \\ 7772)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(12203, \\ 12203)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(10793, \\ 10793)\end{tabular} \\ \hline
\end{tabular}%
}
\end{table}
\end{comment}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{comment}
\begin{table}[!htbp]
\caption{Different Data Dimensions}
\label{tbl:datadim}
\begin{tabular}{|l|p{6mm}|l|l|l|}
\hline
 \textbf{CH}  & \textbf{GW} & \textbf{OS} & \textbf{SS}  & \textbf{FG}  \\ \hline
 36189, 11    & 4020, 11    & 11394, 11   & 22775, 11    & 46064, 11    \\ \hline
18700, 304   & 2906, 304   & 7772, 304   & 12203, 304   & 10793, 304   \\ \hline
18700, 18700 & 2906, 2906  & 7772, 7772  & 12203, 12203 & 10793, 10793 \\ \hline
\end{tabular}
\end{table}
\end{comment}



\begin{comment}
    
\begin{table}[!htbp]
\caption{Different Data Dimensions}
\label{tbl:datadim}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{No} & \textbf{CH} & \textbf{GW} & \textbf{OS} & \textbf{SS} & \textbf{FG} \\ \hline
\textbf{1}  & 36189, 11   & 4020, 11    & 11394, 11   & 22775, 11   & 46064, 11   \\ \hline
\textbf{2}  & 18700, 300  & 2906, 300   & 7772, 300   & 12203, 300  & 10793, 300  \\ \hline
\end{tabular}
\end{table}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[!htbp]
\caption{Different Data Dimensions}
\label{Tbl:DataDim}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{No}        & \textbf{CH} & \textbf{GW} & \textbf{OS} & \textbf{SS} & \textbf{FG} \\ \hline
\multirow{}{}{1} & 36189       & 4020        & 11394       & 22775       & 46064       \\ \cline{2-6} 
                   & 11          & 11          & 11          & 11          & 11          \\ \hline
\multirow{}{}{2} & 18700       & 2906        & 7772        & 12203       & 10793       \\ \cline{2-6} 
                   & 25924       & 5201        & 9415        & 15987       & 24749       \\ \hline
\multirow{}{}{3} & 18700       & 2906        & 7772        & 12203       & 10793       \\ \cline{2-6} 
                   & 3574        & 767         & 1657        & 2661        & 2795        \\ \hline
\multirow{}{}{4} & 18700       & 2906        & 7772        & 12203       & 10793       \\ \cline{2-6} 
                   & 18700       & 2906        & 7772        & 12203       & 10793       \\ \hline
\end{tabular}%
}
\end{table}
\end{comment}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=15cm,height=11cm,trim = {0cm 9cm 0cm 3cm}, clip, keepaspectratio]{Figures/framework.pdf}
    \caption{Framework}\label{fig:framework}
\end{figure*}

\noindent\textbf{Step 3: Calculating \textit{rumor spreaders' intensity score:}}
Tweets' labels only indicate whether a particular tweet is a \textit{rumor} or \textit{non-rumor}. Therefore, in order to identify possible \textit{rumor spreaders}, we calculate a score that indicates the intensity with which users spread \textit{rumors}, which we term as \textit{rumor spreaders' intensity score}.
We compute this score for each user by using the following formula:
    \begin{equation}
    score = \frac{\# \: of\: times\: user\: tweets\: rumor}{Total\: \#\: of\: times\: user\: tweets}
    \end{equation}

where the denominator is calculated by counting the total number of tweets posted by a user, whereas the numerator is calculated by counting the total number of \textit{rumor} tweets posted by a user.
The score range lies between [0, 1], where 0 means not a \textit{rumor spreader}, and 1, indicating possibly a \textit{rumor spreader}. 

In order to validate the effectiveness of this score, we calculate the degree (number of connections) from the user-user reply graph, as shown in Figure \ref{fig:ego_network}.
We observe that the nodes (or users) who are connected to many other nodes (or users), that is, high degree, are more involved in posting \textit{rumor} tweets as compared to nodes (or users) who have a low degree. We then manually check the users with their \textit{rumor spreaders' intensity score} calculated using Equation 1. The score is in line with the degree, which verifies our approach of identifying possible \textit{rumor spreaders}.

%The degree centrality is higher in case of users who are often spreading rumors as compared to users who are not or less spreading the rumors. Thus, it validates the approach of using this score as labels.

To model the problem as a binary classification problem, we put a threshold of $0.5$ to create two classes of users. That is, \textbf{\textit{if the \textit{rumor spreaders' intensity score} is < 0.5, then we assign 0 label (indicating non-rumor spreader class); otherwise, we assign 1 representing the possible rumor spreader class.}}
The reason for choosing this threshold is
based on the observation that the sentiments of the tweets as discussed in Step 1 are positive when the \textit{rumor spreaders' intensity score} is less than 0.5, which is indicative of \textit{non-rumor} spreaders class and vice-versa.
%their tweets' sentiments are positive and vice-versa as discussed in Step 1. 
%Thus, it is an key indicator that this threshold is a valid threshold.
Based on this threshold conversion, Table \ref{Tbl:DescpStat}, column `\# of Spreaders (\%)'  shows the number of possible \textit{rumor spreaders} and \textit{non-rumor spreaders} for each of the five incidents in the dataset.
   
\begin{comment}
    
\begin{table}[!htbp]
\caption{Different Data Dimensions} \label{Tbl:DataDim}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{No} & \textbf{CH}    & \textbf{GW}  & \textbf{OS} & \textbf{SS} & \textbf{FG} \\ \hline
1  & (36189, 
11)    & (4020, 11)   & (11394, 11) & (22775, 11) & (46064, 11)  \\ \hline
2  & (18700, 25924)  & (2906, 5201) & (7772, 9415) & (12203, 15987) & (10793, 15987)
 \\ \hline
3  & (18700, 3573)  & (2906, 766)  & (7772, 1656) & (12203, 2660) & (10793, 2794) \\ 
\hline
4  & (18700, 3574)  & (2906, 767)  & (7772, 1657) & (12203, 2661) & (10793, 2795)
 \\ 
 \hline
5  & (18700, 18700) & (2906, 2906) & (7772, 7772) & (12203, 12203) & (10793, 10793) \\ 
\hline
\end{tabular}
\end{table}
\end{comment}

%\subsection{Transforming the dataset into Suspicious users}\label{sec:TranO2S}
%\fixme{@Shakshi: Here you need to describe how we transform the dataset into something which we used for our analysis.}
%\textbf{Conversion of labels to user's suspicious intensity score - }Labels tells particular tweet is rumor or not. However, in order to detect suspicious users, we need to convert this label to user's suspicious intensity score. The score has been calculated for each user using the below formula - 
\begin{comment}
    \begin{equation}
    score = \frac{Number\: of\: times\: user\: tweets\: rumor}{Total\: number\: of\: times\: user\: tweets}
    \end{equation}

 %The score range lies between [0, 1], where 0 means not a suspicious user and 1 means suspicious user.


%  \textbf{Conversion of scores into labels: }To make this problem \textbf{a classification problem}, the target variable (labels) are calculated like this - 
    
    
    \textbf{\textit{If the user intensity score is < 0.5, then assign 0
    otherwise assign 1}}
s has binary values 0 or 1.
    where, 0 represents not a suspicious user and 1 represents a suspicious user.
    The scores feature that was previously calculated has been removed from the final data.
\end{comment}  

\subsection{Extraction of three sets of features}\label{sec:FeatExt}
In this section, we describe three distinct sets of features that we extract, to be utilized by our machine learning models for predicting possible \textit{rumor spreaders}.
\begin{enumerate}

    \item \textbf{User Features: }
    This
    set of features represents user's profile-based information that includes \textit{followers count}, \textit{favorites count}, and \textit{verified users}.
    
    \item \textbf{Text Features: }
    This feature represents text-related features, such as the \textit{tweet} column in our dataset. 
    We employ popular \textit{Word2Vec} embedding (a specific type of Vector Space Models) \cite{mikolov2013efficient} to convert the tweets into a numeric vector. Specifically, for each unique word in the \textit{tweet}, \textit{Word2Vec} generates its corresponding 300-dimension numeric vector, which is then aggregated in such a way that each sentence represents a 300-dimension vector. 
    %Table \ref{tbl:datadim}, row 2, represents the dimensions after performing word embedding, wherein top value represents the total number of users, and the bottom value represents the total number of features as well as the ground-truth labels in a dataset. %\shakshi{wherein top value represents the total number of users and bottom value represents the total number of features as well as the ground-truth labels in a dataset}. 
    %This embedding's output is sparse in nature as most of the columns (features) are empty, and it  contains %\sout{some} \shakshi{few}
    Besides, we remove few noisy words as well, for instance, aaand, aand, aaaaand using English vocabulary.
    %Thus, we kept only those features which have non-zero values greater than or equal to five. 
    %Table \ref{Tbl:DataDim}, row 3, shows the dimensions of the data after reducing features, wherein top value represents the total number of users and the bottom value represents the total number of features as well as the ground-truth labels in a dataset. 
    %\shakshi{wherein top value represents the total number of uses and bottom value represents the total number of features as well as the ground-truth labels in a dataset}.
    
    \item \textbf{Ego-Network Features}: 
    %\fixme{Can we name it Ego- network Features?}
  To %\sout{add} \shakshi{capture}
  capture the network properties in the data, we %\shakshi{created a feature} \sout{calculate}, \shakshi{known as}
  created a feature which we call as
  \textit{User Importance} (user\_imp) feature. This feature helps in adding the network properties in the dataset by calculating
  the importance of each user with respect to replies it has received. The formula for calculating this feature is as follows:  
    \begin{equation}
    user\_imp = \frac{\#\; of\; replies\; a\; user\; gets}{\#\; of\; replies\; of\; all\; users}
    \end{equation}

    
\end{enumerate}

Figure \ref{fig:framework} summarizes the framework, which we discussed in this Section. Section \ref{sec:Evl} discusses the parameters used by GCN and the results of various approaches.
    
\medskip

==> Shakshi-Rumor_Spreaders-IJCNN(15 jan 21)/Eval.tex <==
\section{Experiments and Result Section}\label{sec:Evl}

In this section, we discuss few of the main hyper-parameter tuning used by our models (Section \ref{sec:parameter_tuning}). Next, we discuss various optimization techniques (Section \ref{sec:Metr}), and lastly, we discuss the results of our approaches (Section \ref{sec:Res}).

As mentioned in Section \ref{sec:intro}, there is a network formation between initiators and responders in terms of tweets. Thus, we use GCN \cite{kipf2016semi}, a type of GNN technique, which can exploit both the network structure and features (such as \textit{tweets, followers count}). In particular, we perform a binary classification for identifying if a specific Twitter user is possibly involved in \textit{rumor} spreading or not. In addition, we compare GCN with other baseline approaches (SVM, RF, and LSTM).

\subsection{Hyper-Parameters tuning}\label{sec:parameter_tuning}

Table \ref{tbl:parameter-tuning} shows the values for
various hyper-parameter settings that are chosen for fine-tuning the models for improving the performance. Here, we have specified few of the main hyper-parameters only.
For instance, 
SVM has a hyper-parameter, \textit{kernel},
which is a function that finds the similarity score between two data points even from the high dimensional input space in order to find the optimal hyperplane.
RF has a hyper-parameter known as, \textit{number of trees in forest} that specifies how many trees should be formed so that they can be used as a parallel estimators in order to make final prediction.
The rest of the hyper-parameters are specific %\sout{for} \shakshi{to} 
to the neural networks (for both LSTM and GCN). The \textit{number of layers in a network} represents the total number of layers used in a model, \textit{number of channels in each layer} represents the total number of output neurons to be used in a layer, \textit{drop out layer} 
is used 
to
avoid overfitting of the data. The \textit{activation function} decides which neuron to activate for the next layer in the network, \textit{number of epochs} refers to the number of iterations the neural network model is to be trained for. The \textit{loss function} is used for refining the model after every epoch.
%The values in the table specify the type of hyper-parameter used in the model. 
%\st{However,} \fixme{wrong usage of "however"}. \fixme{add - The} 
The \textit{NA} values in the table refer to Not Applicable.
    
\begin{table}[!htbp]
\centering
\caption{Hyper-Parameters Tuning of models}
\label{tbl:parameter-tuning}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Parameters\textbackslash\\ Models\end{tabular}} & \textbf{SVM}                                                     & 
\textbf{RF}                                                     & 
\textbf{LSTM}                                                   & \textbf{GCN}                                                   \\ \hline
\textbf{Kernel}                                                                         & \begin{tabular}[c]{@{}l@{}}radial basis \\ function\end{tabular} & NA        & NA                                                      & NA                                                             \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}\# of trees \end{tabular}} & NA     & 100                                                            & 2                                                               & 2                                                              \\ \hline

\textbf{\# of layers}                                                                         & \begin{tabular}[c]{@{}l@{}}NA \end{tabular} & NA & 2                                                             & 2
\\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}\# of channels\\ in first layer\end{tabular}} & NA           & NA                                                               & 32                                                              & 32                                                             \\ \hline

\textbf{\begin{tabular}[c]{@{}l@{}}\# of channels \\ in second layer\end{tabular}}      & NA    & NA                                                           & 2                                                               & 2                                                              \\ \hline
\textbf{Drop out layer}                                         & NA                        & NA                                                               & 0                                                              & 2                                                              \\ \hline
\textbf{\# of Epochs}                                                                      & NA      & NA                                                         & 300                                                             & 300                                                            \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Activation \\ function\end{tabular}}                 & NA        & NA                                                       & sigmoid                                                         & sigmoid                                                        \\ \hline
\textbf{Loss function}                                                                  & average & hinge                                                            & \begin{tabular}[c]{@{}l@{}}binary cross \\ entropy\end{tabular} & \begin{tabular}[c]{@{}l@{}}binary cross\\ entropy\end{tabular} \\ \hline
\end{tabular}
\end{table}
   
    Apart from the Table \ref{tbl:parameter-tuning} hyper-parameters, GCN model takes two additional inputs - graph adjacency matrix and nodes' features matrix. 
    The graph adjacency matrix stores the nodes' neighbors information in a $Z$X$Z$ matrix, where $Z$
    represents the total number of nodes (users) in the dataset. The nodes' features matrix $Z$X$F$ is the final matrix of the preprocessing step, where $Z$ represents the number of nodes and $F$ is the size of total features.
    As already mentioned, Table \ref{tbl:datadim}, column `Rumor Spreaders', shows the dimensions of the nodes' features matrix for each of the incident. 
    Specifically, each cell
    values represents the nodes, $Z$ and the features, $F$ where $F$ represents the features (attributes) such as \textit{followers count}, word embedding of tweet, \textit{user\_imp}. 
    In addition, the dimensions of the adjacency matrix are shown in \ref{tbl:datadim}, column `Adjacency Matrix',
    wherein each cell values represents the total number of users in a dataset.
    After providing required inputs to GCN, the model is trained to predict possible \textit{rumor} and \textit{non-rumor spreaders}.
    %Following is the propagation rule for every layer in the network. This rule is inspired from first-order approximation of localized spectral filters on graphs \cite{kipf2016semi}.
    %\begin{equation}
    %\boldsymbol{H^{(l+1)} = \sigma (\Tilde{D}^{-\frac{1}{2} }  \: \Tilde{A}\:  \Tilde{D}^{-\frac{1}{2}}\:  H^{(l)} \: W^{(l)})},
  %  \end{equation}
   
    %\shakshi{Need to write dimension of hidden layer, change mathematical notations.}
   % where, \textit{H\textsuperscript{(l+1)}} 
    %represents the current hidden layer, \textit{\(\sigma\)}
    %is the non-linear activation function, \textit{\(\Tilde{D}\)\textsuperscript{-0.5}}  is the normalized degree matrix, 
    %\textit{\(\Tilde{A}\)}
    %represents symmetric adjacency matrix with self-connections, \textit{W\textsuperscript{(l)}} is the learnable weight matrix parameter of previous hidden layer.
  
    %At layer \textit{l = 0},
    %\begin{equation*}
     %   \boldsymbol{H^{(0)} \: = X}   
    %\end{equation*}
    %where \textit{X} represents the nodes' features matrix. %\shakshi{of dimension \textit{$N$X$F$}}.
    %The last layer is used for classification.
    In order to predict possible \textit{rumor spreaders}, the nodes have labels as 0
    (\textit{non-rumor spreader}) or 1 (possibly a \textit{rumor spreader}). 
    In Section \ref{sec:Res}, we discuss results of all the machine learning approaches.


\subsection{Optimization Techniques}\label{sec:Metr}

As part of the optimization, we perform following steps -

\begin{enumerate}
    \item \textbf{Cross Validation:} To ensure the effectiveness of our model and to avoid overfitting of data, we perform K-Fold cross-validation on our dataset where \textit{K = 5}. To avoid the class imbalance problem in \textit{Charlie} incident, we use Stratified K-Fold.

    \item \textbf{Standardization: }All the features are standardized before training the machine learning model.
    \item \textbf{Feature Importance: }In addition to the above two techniques, three feature selection techniques, namely, \textit{Chi-Square, Information Gain, Gain Ratio} are applied to each of the five incidents of rumor spreaders dataset to check whether each feature is correlated with the target variable. %Results shows that all of the features being mentioned in Section \ref{sec:ds} are correlated with the target variable. Thus, we consider all of the features and feed it into the model.
    Table \ref{tbl:feature} depicts the p-values of three feature selection techniques. For all the features, p-value < 0.05 which shows that these features are important in predicting possible \textit{rumor spreaders}. Thus, we consider all the features in our experiments.
\end{enumerate}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!htbp]
\caption{Feature Selection Techniques (values in the cells indicates their corresponding p-values)}
\label{tbl:feature}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Features}& \textbf{Chi-Square} & \textbf{Information Gain} & \textbf{Gain Ratio} \\ \hline
\textbf{followers count}                           & 5.28e-05            & 4.62e-07                  & 8.56e-09            \\ \hline
\textbf{favorites count}                           & 8.66e-17            & 11.65e-22                 & 5.56e-11            \\ \hline
\textbf{verified users}                            & 2.26e-10            & 1.44e-05                  & 3.67e-07            \\ \hline
\textbf{user importance}                           & 7.87e-20            & 9.93e-23                  & 7.83e-26            \\ \hline
\end{tabular}
\end{table}

\begin{table}[!htbp]
\centering
\caption{Metrics performance of different models}
\label{Tbl:gw}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{S.No.} & \textbf{Metrics} & \textbf{SVM} & \textbf{RF} & \textbf{LSTM} & \textbf{GCN} \\ \hline
\multicolumn{6}{|c|}{\textbf{\textcolor{blue}{Charlie}}} \\ \hline
1 & \textbf{Accuracy}          &  0.748             & 0.760 &      0.671        &    \textbf{0.790}         \\ \hline
2 & \textbf{Precision}          &    0.748          & 0.758 &   0.571            &     \textbf{0.790}         \\ \hline
3 & \textbf{Recall}             &   0.748           & 0.628 &          0.571     &       \textbf{0.790}       \\ \hline
4 & \textbf{F1-Score}        &     0.853        & 0.840  &         0.778      &       \textbf{0.864}       \\ \hline
5 & \textbf{AUC-ROC}     &     0.600        & 0.600 &       0.570        &        \textbf{0.690}      \\ \hline
\multicolumn{6}{|c|}{\textbf{\textcolor{blue}{German}}} \\ \hline
6 & \textbf{Accuracy}           & 0.552             & 0.567 &       0.541        &    \textbf{0.715}          \\ \hline
7 & \textbf{Precision}          &  0.553 & 0.567            &         0.541      &      \textbf{0.717}        \\ \hline
8 & \textbf{Recall}             & 0.552        & 0.567     &         0.541      &      \textbf{0.716}        \\ \hline
9 & \textbf{F1-Score}         &   0.572           & 0.567 &        0.546       &       \textbf{0.709}       \\ \hline
10 & \textbf{AUC-ROC}      & 0.552             & 0.566 &         0.540      &       \textbf{0.720}       \\ \hline
\multicolumn{6}{|c|}{\textbf{\textcolor{blue}{Ottawa}}} \\ \hline
11 & \textbf{Accuracy}           &     0.567         & 0.565 &     0.552          &      \textbf{0.675}        \\ \hline
12 & \textbf{Precision}          & 0.567             & 0.565 &      0.552         &      \textbf{0.681}        \\ \hline
13 & \textbf{Recall}             &    0.566          & 0.565 &     0.552          &     \textbf{0.677}         \\ \hline
14 & \textbf{F1-Score}         &      0.578  & 0.569      &        0.559       &       \textbf{0.655}       \\ \hline
15 & \textbf{AUC-ROC}      &      0.566        & 0.566 &         0.550      &        \textbf{0.680}      \\ \hline
\multicolumn{6}{|c|}{\textbf{\textcolor{blue}{Sydney}}} \\ \hline
16 & \textbf{Accuracy}           &     0.618         &0.639 &     0.561          &      \textbf{0.655}        \\ \hline
17 & \textbf{Precision}          & 0.565             & 0.606 &      0.541         &      \textbf{0.655}        \\ \hline
18 & \textbf{Recall}             &    0.520          & 0.579 &     0.542        &     \textbf{0.664}         \\ \hline
19 & \textbf{F1-Score}         &      \textbf{0.751} &0.740        &        0.638       &       0.690       \\ \hline
20 & \textbf{AUC-ROC}      &      0.618        & 0.638 &         0.540      &        \textbf{0.660}      \\ \hline
\multicolumn{6}{|c|}{\textbf{\textcolor{blue}{Ferguson}}} \\ \hline
21 & \textbf{Accuracy}           &     0.652         & 0.675 &     0.585          &      \textbf{0.705}        \\ \hline
22 & \textbf{Precision}          & 0.598             & 0.634 &      0.549        &      \textbf{0.671}        \\ \hline
23 & \textbf{Recall}             &    0.519          & 0.589 &     0.549         &     \textbf{0.658}         \\ \hline
24 & \textbf{F1-Score}         &     0.782       & 0.778 &        0.676       &       \textbf{0.783}       \\ \hline
25 & \textbf{AUC-ROC}      &      0.652        & \textbf{0.674} &         0.550      &        0.660      \\ \hline
\end{tabular}
\end{table}
\subsection{Results}\label{sec:Res}
In this section, we discuss the micro and macro-analysis of our evaluation for all the incidents using five metrics.

\noindent \textbf{{1. Macro-Analysis}}\label{sec:macro}: Table \ref{Tbl:gw} provides the macro-averaged results of our machine learning models for all the five metrics for \textit{Charlie}, \textit{German}, \textit{Ottawa}, \textit{Sydney}, and \textit{Ferguson} respectively. In general, GCN outperforms other classifiers in all the five metrics. SVM and RF perform better than LSTM in most of the metrics. Considering per incident evaluations, the results of \textit{German} incident outperforms with a significant margin, whereas \textit{Charlie} results exceed with a small margin. In spite of using Stratified K-Fold, the class imbalance problem might have affected the \textit{Charlie} results. 


\begin{comment}

\begin{table}[!htbp]
\centering
\caption{Charlie hebdo}
\label{Tbl:ch}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Metrics/Classifers} & \textbf{SVM} & \textbf{RF} & \textbf{LSTM} & \textbf{GCN} \\ \hline
\textbf{Accuracy}          &  0.748             & 0.760 &      0.671        &    \textbf{0.790}         \\ \hline
\textbf{Precision}          &    0.748          & 0.758 &   0.571            &     \textbf{0.790}         \\ \hline
\textbf{Recall}             &   0.748           & 0.628 &          0.571     &       \textbf{0.790}       \\ \hline
\textbf{F1-Score}        &     0.853        & 0.840  &         0.778      &       \textbf{0.864}       \\ \hline
\textbf{AUC-ROC Score}     &     0.600        & 0.600 &       0.570        &        \textbf{0.690}      \\ \hline
\end{tabular}
\end{table}
\end{comment}

\begin{comment}
\begin{table}[!htbp]
\centering
\caption{Ottawa shooting}
\label{Tbl:os}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Metrics/Classifers} & \textbf{SVM} & \textbf{RF} & \textbf{LSTM} & \textbf{GCN} \\ \hline
\textbf{Accuracy}           &     0.567         & 0.565 &     0.552          &      \textbf{0.675}        \\ \hline
\textbf{Precision}          & 0.567             & 0.565 &      0.552         &      \textbf{0.681}        \\ \hline
\textbf{Recall}             &    0.566          & 0.565 &     0.552          &     \textbf{0.677}         \\ \hline
\textbf{F1-Score}         &      0.578  & 0.569      &        0.559       &       \textbf{0.655}       \\ \hline
\textbf{AUC-ROC Score}      &      0.566        & 0.566 &         0.550      &        \textbf{0.680}      \\ \hline
\end{tabular}
\end{table}

\begin{table}[!htbp]
\centering
\caption{Sydney siege} \PS{These 2 tables might go up when the text is cleaned after removing comments.
}
\label{Tbl:ss}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Metrics/Classifers} & \textbf{SVM} & \textbf{RF} & \textbf{LSTM} & \textbf{GCN} \\ \hline
\textbf{Accuracy}           &     0.618         &0.639 &     0.561          &      \textbf{0.655}        \\ \hline
\textbf{Precision}          & 0.565             & 0.606 &      0.541         &      \textbf{0.655}        \\ \hline
\textbf{Recall}             &    0.520          & 0.579 &     0.542        &     \textbf{0.664}         \\ \hline
\textbf{F1-Score}         &      \textbf{0.751} &0.740        &        0.638       &       0.690       \\ \hline
\textbf{AUC-ROC Score}      &      0.618        & 0.638 &         0.540      &        \textbf{0.660}      \\ \hline
\end{tabular}
\end{table}
\begin{table}[!htbp]
\centering
\caption{Ferguson}
\label{Tbl:fg}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Metrics/Classifers} & \textbf{SVM} & \textbf{RF} & \textbf{LSTM} & \textbf{GCN} \\ \hline
\textbf{Accuracy}           &     0.652         & 0.675 &     0.585          &      \textbf{0.705}        \\ \hline
\textbf{Precision}          & 0.598             & 0.634 &      0.549        &      \textbf{0.671}        \\ \hline
\textbf{Recall}             &    0.519          & 0.589 &     0.549         &     \textbf{0.658}         \\ \hline
\textbf{F1-Score}         &     0.782       & 0.778 &        0.676       &       \textbf{0.783}       \\ \hline
\textbf{AUC-ROC Score}      &      0.652        & \textbf{0.674} &         0.550      &        0.660      \\ \hline
\end{tabular}
\end{table}

\end{comment}
\begin{comment}
\begin{figure*}[!htbp]
    \begin{right}
    \subfigure(a)
    {\includegraphics[width=0.18\textwidth]{Figures/c_acc.png}}
    \subfigure(b){\includegraphics[width=0.18\textwidth]{Figures/c_p.png}} 
    \subfigure(c){\includegraphics[width=0.18\textwidth]{Figures/c_r.png}}
    \subfigure(d){\includegraphics[width=0.18\textwidth]{Figures/c_f.png}}
    \subfigure(e){\includegraphics[width=0.18\textwidth]{Figures/c_auc.png}}
    \end{right}
    \caption{ Performance of GCN model on Charlie hebdo under five-fold cross validation}\label{fig:ch}
\end{figure*}
\begin{figure*}[!htbp]
    \begin{right}
    \subfigure(a)
    {\includegraphics[width=0.18\textwidth]{Figures/g_acc.png}}
    \subfigure(b){\includegraphics[width=0.18\textwidth]{Figures/g_p.png}} 
    \subfigure(c){\includegraphics[width=0.18\textwidth]{Figures/g_r.png}}
    \subfigure(d){\includegraphics[width=0.18\textwidth]{Figures/g_f.png}}
    \subfigure(e){\includegraphics[width=0.18\textwidth]{Figures/g_auc.png}}
    \end{right}
    \caption{ Performance of GCN model on German wings crash under five-fold cross validation}\label{fig:ger}
\end{figure*}



\begin{figure*}[!htbp]
    \begin{right}
    \subfigure(a)
    {\includegraphics[width=0.18\textwidth]{Figures/o_acc_plot.pdf}}
    \subfigure(b){\includegraphics[width=0.18\textwidth]{Figures/o_p_plot.pdf}} 
    \subfigure(c){\includegraphics[width=0.18\textwidth]{Figures/o_r_plot.pdf}}
    \subfigure(d){\includegraphics[width=0.18\textwidth]{Figures/o_f_plot.pdf}}
    \subfigure(e){\includegraphics[width=0.18\textwidth]{Figures/o_auc_plot.pdf}}
    \end{right}
    \caption{Performance of GCN model on Ottawa shooting under five-fold cross validation}\label{fig:ottawa}
\end{figure*}




\begin{figure*}[!htbp]
    \begin{right}
    \subfigure(a)
    {\includegraphics[width=0.18\textwidth]{Figures/s_acc.png}}
    \subfigure(b){\includegraphics[width=0.18\textwidth]{Figures/s_p.png}} 
    \subfigure(c){\includegraphics[width=0.18\textwidth]{Figures/s_r.png}}
    \subfigure(d){\includegraphics[width=0.18\textwidth]{Figures/s_f.png}}
    \subfigure(e){\includegraphics[width=0.18\textwidth]{Figures/s_auc.png}}
    \end{right}
    \caption{ Performance of GCN model on Sydney siege under five-fold cross validation}\label{fig:sydney}
\end{figure*}


\begin{figure*}[!htbp]
    \begin{right}
    \subfigure(a)
    {\includegraphics[width=0.18\textwidth]{Figures/f_acc.png}}
    \subfigure(b){\includegraphics[width=0.18\textwidth]{Figures/f_p.png}} 
    \subfigure(c){\includegraphics[width=0.18\textwidth]{Figures/f_r.png}}
    \subfigure(d){\includegraphics[width=0.18\textwidth]{Figures/f_f.png}}
    \subfigure(e){\includegraphics[width=0.18\textwidth]{Figures/f_auc.png}}
    \end{right}
    \caption{ Performance of GCN model on Ferguson under five-fold cross validation}\label{fig:fer}
\end{figure*}




\begin{figure*}[!htbp]
     \subfloat[Charlie hebdo\label{subfig-1:charlie}]{%
       \includegraphics[width=0.20\textwidth]{Figures/f_acc.png}
     }
       \subfloat[German wings crash\label{subfig-1:german}]{%
       \includegraphics[width=0.20\textwidth]{Figures/f_p.png}
     }
     \subfloat[Ottawa shooting\label{subfig-2:ottawa}]{%
       \includegraphics[width=0.20\textwidth]{Figures/f_r.png}
     }
      \subfloat[Sydney siege\label{subfig-2:sydney}]{%
       \includegraphics[width=0.20\textwidth]{Figures/f_f.png}
     }
      \subfloat[Ferguson\label{subfig-2:ferguson}]{%
       \includegraphics[width=0.20\textwidth]{Figures/f_auc.png}
     }
     \caption{Performance of AUC-ROC Curve on five incidents}
     \label{fig:aucroc}
   \end{figure*}
\end{comment}

\begin{figure*}[ht!]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
{} & Accuracy & Precision & Recall & F1-Score & AUC-ROC\\\hline
\rotatebox{90}{\hspace{4mm}Charlie}
&
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/c_acc_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/c_p_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/c_r_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/c_f_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/c_auc_plot.pdf}}\\\hline


\rotatebox{90}{\hspace{4mm}German} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/g_acc_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/g_p_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/g_r_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/g_f_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/g_auc_plot.pdf}}\\\hline



\rotatebox{90}{\hspace{7mm}Ottawa} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/o_acc_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/o_p_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/o_r_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/o_f_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/o_auc_plot.pdf}}\\\hline

\rotatebox{90}{\hspace{6mm}Sydney} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/s_acc_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/s_p_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/s_r_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/s_f_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/s_auc_plot.pdf}}\\\hline



\rotatebox{90}{\hspace{5mm}Ferguson} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/f_acc_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/f_p_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/f_r_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/f_f_plot.pdf}} &
\subfloat{\includegraphics[width=0.35\columnwidth]{Figures/f_auc_plot.pdf}}\\\hline

\end{tabular}
\caption{Performance of GCN model under five-fold cross validation for all the incidents}
\label{fig:cv}
\end{figure*}

\begin{figure*}[!htbp]
     \subfloat[Charlie \label{subfig-1:charlie}]{%
       \includegraphics[width=0.20\textwidth]{Figures/ch.png}
     }
       \subfloat[German  \label{subfig-1:german}]{%
       \includegraphics[width=0.20\textwidth]{Figures/ger.png}
     }
     \subfloat[Ottawa \label{subfig-2:ottawa}]{%
       \includegraphics[width=0.20\textwidth]{Figures/ot.png}
     }
      \subfloat[Sydney \label{subfig-2:sydney}]{%
       \includegraphics[width=0.20\textwidth]{Figures/ss.png}
     }
      \subfloat[Ferguson\label{subfig-2:ferguson}]{%
       \includegraphics[width=0.20\textwidth]{Figures/fer.png}
     }
     \caption{Performance of AUC-ROC Curve on all the five incidents}
     \label{fig:aucroc}
   \end{figure*}

\noindent \textbf{{2. Micro-Analysis}}\label{sec:micro}: Figure \ref{fig:cv} shows the micro-performance of each of the approaches under five metrics for all the incidents in our dataset. Specifically, the x-axis represents the fold number under five-fold cross-validation, whereas the y-axis represents the metrics used for evaluation. To summarize, each incident consisting of five plots depicting Accuracy, Precision, Recall, F1-Score, and AUC-ROC Score for each fold. It can be seen from the plots that, in general, the GCN approach is performing better than the baseline models. However, GCN approach on \textit{German} and \textit{Ottawa} incidents performed significantly better compared to the other two approaches.
This clearly implies that the GCN approach is a natural fit for our problem statement.

Furthermore, we plot the AUC-ROC plot for each of the incidents to understand the micro-performance of the algorithm at different thresholds. Figure \ref{fig:aucroc} shows the AUC-ROC Curve for \textit{Charlie}, \textit{German}, \textit{Ottawa}, \textit{Sydney}, and \textit{Ferguson} respectively. It can be noticed that SVM, RF, and LSTM perform little better than the random model, whereas GCN is better with a good margin. However, RF performs better than the other two baselines in the case of the \textit{Ferguson} incident. Besides, the GCN approach performs well on lower thresholds for \textit{German}, \textit{Ottawa}, and \textit{Sydney}. In contrast, the reverse is the case for \textit{Charlie}, and \textit{Ferguson} indicating the reasons, higher values of Accuracy, Precision, Recall, and F1-Score than AUC-ROC values for the \textit{Charlie} and higher values of Accuracy, Precision, and F1-Score
than AUC-ROC values for the \textit{Ferguson} incident. In all cases, the results are indicative that GCN is able to exploit the relation among the initiator's tweet and its responders, which helped it to perform better.

==> Shakshi-Rumor_Spreaders-IJCNN(15 jan 21)/background.tex <==
\section{Graph Convolutional Network}\label{sec:gcn}
\medskip

\sout{GNN is a new and popular branch of machine learning that operates on non-Euclidean data. Data that inherently forms a network is a good fit for GNN. For instance, citation network, social network,  protein-protein interaction network, to name a few. Unlike network embedding approaches (such as DeepWalk \cite{perozzi2014deepwalk}, node2vec \cite{grover2016node2vec}), GNN captures the graph properties. In particular node attributes and can be generalized to unseen nodes (graphs) as well. There exist multiple variants of GNN such as Graph Convolution, Graph Autoencoder, Graph Recurrent Neural Network.
    
Graph Convolution is a %\sout{specific kind} \shakshi{particular type} 
particular type of GNN and %\sout{the Graph Convolution} \shakshi{its} 
its framework is inspired from Convolutional Neural Network \cite{krizhevsky2012imagenet}. Based on kernel selection, Graph Convolution can be bifurcated into two classes, spectral based and spatial based. In spectral based kernel selection, inputs are transformed into the spectral domain with the help of eigenvalue decomposition wherein the kernel, and the transformed input gets convolved. Furthermore, the transformed inputs bring back to the original domain in order to be used by next layer in the network. In comparison, spatial based kernel selection aggregates the information of neighboring nodes by itself in order to maintain the topology of the network. The aggregated information fetched from the previous layer is then passed to the following layer in network \cite{wu2020comprehensive, hamilton2017representation}. This idea of message passing is inspired from Recurrent Neural Network (RNN).
    
    
    Graph Convolutional Network (GCN) \cite{kipf2016semi} is a spectral based two-layer network designed for the semi-supervised node classification task. The inputs to GCN are features matrix of dimension \textit{$N$X$F$} and symmetric adjacency matrix of dimension \textit{$N$X$N$}, where \textit{N} is the number of nodes in the graph and \textit{F} is the number of features.
    
    Following is the propagation rule for every layer in the network. This rule is inspired from first-order approximation of localized spectral filters on graphs \cite{kipf2016semi}.
    \begin{equation}
    \boldsymbol{H^{(l+1)} = \sigma (\Tilde{D}^{-0.5}   \: \Tilde{A}\:  \Tilde{D}^{-0.5}\:  H^{(l)} \: W^{(l)})},
    \end{equation}
   
    %\shakshi{Need to write dimension of hidden layer, change mathematical notations.}
    where, \textit{H\textsuperscript{(l+1)}} 
    represents the current hidden layer, \textit{\(\sigma\)}
    is the non-linear activation function, \textit{\(\Tilde{D}\)\textsuperscript{-0.5}}  is the normalized degree matrix, 
    \textit{\(\Tilde{A}\)}
    represents symmetric adjacency matrix with self-connections, \textit{W\textsuperscript{(l)}} is the learnable weight matrix parameter of previous hidden layer.
  
    At layer \textit{l = 0},
    \begin{equation*}
        \boldsymbol{H^{(0)} \: = X}   
    \end{equation*}
    where \textit{X} represents the nodes' features matrix %\shakshi{of dimension \textit{$N$X$F$}}.
    of dimension \textit{$N$X$F$}.
    The last layer is used for classification. Number of nodes in the last layer depend on number of classes. After building the model, the weights are trained using stochastic gradient descent algorithm  until either a loss function is minimized to  a certain defined level or model completed a specified number of iterations (or epochs).
    }

==> Shakshi-Rumor_Spreaders-IJCNN(15 jan 21)/conclusion.tex <==
\section{Conclusion and Future Work}\label{sec:concl}
Identifying possible \textit{rumor spreaders} is crucial as it has been shown that they are the potential sources of \textit{rumor} propagation \cite{volkova2017separating}. In this work, we use the \textbf{PHEME} dataset to identify
%focused on identifying 
possible \textit{rumor spreaders} %applying transformation steps to the rumor dataset in order to identify possible \textit{rumor spreaders} 
using a weak supervised learning approach. We model this problem as binary classification task by
applying various machine learning models to the transformed rumor spreaders dataset. 
%We evaluated our approach on the \textbf{PHEME} dataset. 
Our results show that  GCN  (compared  to baseline  models)  is  able  to  perform better (to raise red flags for possible \textit{rumor spreaders}) by exploiting relationships of possible \textit{rumor spreaders} who could blend well with \textit{non-rumor spreaders}.
%Our results show that GCN (compared to baseline models) is able to perform better by exploiting relationships of possible \textit{rumor spreaders} who could blend well with \textit{non-rumor spreaders}. 
The overall performance of the GCN shows the effectiveness of this approach.
%leading to better performance which shows the effectiveness of this approach. %Our aim was to show the ability of the network to show relationships between these users who could blend well with non-suspicious users. 
We would like to improve this work through the following multiple plans:
\begin{enumerate}
    \item \textbf{Multiclass problem: }In our present work, we transformed the dataset to study it as a binary classification problem. However, in our extended work, we would like to model this problem as a multiclass prediction to minimize the loss in transformation. %or as a regression
    \item \textbf{Additional datasets: }%\sout{In addition to applying the approach on the other two incidents in the PHEME datasets,} 
    The transformation of \textit{rumor} dataset into rumor spreaders dataset may induces bias. To overcome that,
    we would like to apply this framework on datasets containing all the tweets posted by a user as opposed to only collecting tweets by a specific topic. % for our evaluation%\sout{we also plan to include additional datasets in our evaluation}.
    \item \textbf{New algorithms: }To extend our research, we plan to apply other graph neural network techniques that works well on unseen graph structures (inductive learning) such as Graph Attention Networks \cite{velivckovic2017graph}, GraphSage \cite{wu2020comprehensive}. 
    %\fixme{are you sure GraphSage is a GCN type or ? if we are confuse, we can remove Graphsage?}
\end{enumerate}
\section{ACKNOWLEDGMENT}
This  research  is  funded  by H2020 project, SoBigData++, and CHIST-ERA project SAI.
%\section{ Acknowledgments}

==> Shakshi-Rumor_Spreaders-IJCNN(15 jan 21)/intro.tex <==
\section{Introduction}\label{sec:intro}

%Online Social Media (OSM) platforms, initially developed for connecting individuals across the globe for better communication, have turned into a medium for diffusing news (or information) \cite{kwak2010twitter}. On one side, these platforms offer a place for the expression of views. However, on the flip side, these platforms have not been able to regulate the spread of misinformation. According to \cite{mitnews}, false information propagates six times faster than the true news on these platforms, which can result in panic, fear, and financial loss to society \cite{zubiaga2018detection}. Thus, it is important to control misinformation propagation before it spreads to the masses.

Online  Social  Media  (OSM)  platforms,  initially  developed for  connecting  individuals have become a hotbed for users who spread misinformation  regularly  by  exploiting  the  connectivity  and globality  of  these  platforms \cite{kwak2010twitter}. On  one  side,  these  platforms  offer  a place  for  the  expression  of  views.  However,  on  the  flip  side, these  platforms  have  not  been  able  to  regulate  the  spread  of misinformation. According to \cite{mitnews}, false information propagates six times faster than the true news on these platforms, which can result in panic, fear, and financial loss to society \cite{zubiaga2018detection}. Thus, it is important to control misinformation propagation before it spreads to the masses. However, it is not a trivial task to identify such users  as  they  blend  very  well  by  creating  many  connections with users who are not involved in spreading misinformation activities \cite{fire2014friend}.

%OSM platforms have become a hotbed for users who spread misinformation regularly by exploiting the connectivity and globality of these platforms \cite{kwak2010twitter}. \shakshi{This line is same as above paragraph. Should we combine both these paragraphs?}
%However, it is not a trivial task to identify such users as they blend very well by creating many connections with users who are not involved in spreading misinformation activities \cite{fire2014friend}. 

%This work deals with \shakshi{tackling misinformation especially identifying possible \textit{rumor spreaders} on Twitter}.
%\PS{A rumor is a piece of information whose validity is in doubt at the time of posting. In other words, there is a doubt whether the information being posted is true or false.}
%Next, we define \textit{rumor spreaders} as those users who are often engaged in spreading the rumors \cite{zubiaga2018detection}. 
%\fixme{this kind of text should go in future work. We will discuss this in call to understand why you wrote this.}\PS{Please note that this work is the preliminary work to identify possible \textit{rumor spreaders} utilizing tweets information only.
%In addition, we use the term 'possible' in our work to state that it is likely that the user could be a \textit{rumor spreader}.}

Misinformation can be categorized into two main types. The first one is the \textit{fake news}, the news which is certainly not true. The second one is the \textit{rumors}, a piece of information whose validity is in doubt at the time of posting. In other words, there is a doubt whether the information being posted is true or false. In this work, we focus on identifying the ``possible'' \textit{rumor spreaders}. We define \textit{rumor spreaders} as those users who are often engaged in spreading the rumors \cite{zubiaga2018detection}, and the term ``possible'' in our work points to the fact that it is very likely that the user could be a \textit{rumor spreader}.

In the past, researchers have proposed various techniques for identifying suspicious or malicious users involved in the spread of misinformation on OSM platforms such as Twitter. These works include analyzing the user profiles' information \cite{benevenuto2010detecting, thomas2013trafficking}, observing user activity patterns across a specific time window \cite{gupta2017towards, gurajala2015fake}, tracking the profiles through the usage of a smartphone's battery \cite{salehan2013social}. Furthermore, few additional %\sout{some other}
approaches %\sout{used} \shakshi{utilized}
utilized graph-based techniques \cite{cao2012aiding} and multi-modal feature exploitation \cite{jiang2014detecting} for the detection of malicious profiles.
 
Identifying possible \textit{rumor spreaders} is important, as they could be the potential source of misinformation propagation. Curbing on such users means controlling the misinformation diffusion as well. However,
this problem has not acquired significant
attention in contrast to detecting \textit{rumors} or \textit{fake news}. This is primarily due to the lack of an annotated dataset about \textit{rumor spreaders} \cite{han2019neural}.
Thus, identifying possible \textit{rumor spreaders} is challenging in many aspects, which is the theme of this research work.

In this paper, we use the \textbf{PHEME} dataset, which
contains \textit{rumor} and \textit{non-rumor} tweets about five incidents, that is, i) \textit{Charlie hebdo}, ii) \textit{German wings crash}, iii) \textit{Ottawa shooting}, iv) \textit{Sydney siege}, and v) \textit{Ferguson} occurred between 2014 and 2015. %This dataset consists of labeled information about tweets, that is, whether \PS{the information posted on Twitter is a rumor or not. 
%\sout{We then transform this \textbf{PHEME} tweets dataset into rumor spreaders dataset using weak supervised learning and other techniques as well}
%\PS{Is this line ok?-------
%In order to transform the tweets dataset into rumor spreaders dataset, one of the techniques we utilize is the weak supervised learning technique.
In order to transform the tweets dataset into a rumor spreaders dataset\footnote{Code and data is available at - https://github.com/shakshi12/RumourGNN}, we explore the sentiments of the tweets and calculate the \textit{rumor spreaders' intensity score} (that is, how often a user posts \textit{rumor} tweets). In addition, we also utilize the weak supervised learning approach,
%By leveraging techniques such as weak supervised learning, we transform this dataset into rumor spreaders dataset. }
%\fixme{Suggestion -- By leveraging the weak supervised learning technique [citation? reuse some citation], we transform \st{this} \fixme{tweet} dataset into rumor spreaders dataset}. 
%Weak supervised learning 
which is a branch of machine learning used to label the un-annotated data using few or noisy labels in order to avoid the expensive task of manual annotation of the data \cite{weaksupervision}. 
Please note that the labels that are generated using this approach are the \textit{near ground-truth} labels. Thus, we use the term `possible' for rumor spreaders dataset.

%Please note that using these mentioned approaches, the labels we get for each user is the \textit{near ground-truth} labels.
%\st{Then, the transformed dataset is applied to various machine learning classifiers, especially, GCN which shows that GCN is a natural fit for our problem. This is due to the fact that the dataset itself contains inherent network as will be discussed in later section.}

%\fixme{suggestion for your blue blue -- rumor  spreaders’  dataset using  Vector  Space  model, an information retrieval  technique for doing bla bla? Next, for annotating the ground truth, we use weak supervised learning approach. [can we explain in 1/2 lines about it?]. We then apply various machine learning approaches. In particular, we employ Graph Convolution Network approach we exploiting the network structure?? }
After the data transformation step, we leverage the following three distinct features for classifying possible \textit{rumor spreaders}:
\begin{enumerate}
\item \textbf{User Features: }This includes users' features such as \textit{number of followers, number of favorites}.

\item \textbf{Text Features: }We exploit users' tweets as a second set of features.% \fixme{may be we can remove the second line .. does not make such sense to put it here.} In particular, \PS{ we employ one of the popular Vector Space Models for constructing numerical vectors. }

\item \textbf{Ego-Network Features:} 
We also explore the network of users who posted the tweets and the users who respond to those tweets. 
We illustrate this
%We illustrate the same 
using Figure \ref{fig:ego_network}, wherein the central node I is a node who has posted a tweet, which we refer to as initiator user and the nodes \textbf{R1, R2, R3}, and \textbf{R4} are the responder users who have replied to the user \textbf{I}'s tweet. The weights on the edges correspond to the number of times user \textbf{I}, and responder user interacted with each other. Based on our dataset, we are only able to create a one-hop network (ego-network) comprising of initiator user and its responders.
%\shakshi{As it can be seen from Figure \ref{fig:ego_network}, the central node \textbf{I} is the initiator user, who initiated the tweet and the nodes \textbf{R1, R2, R3} and \textbf{R4} are the responder users who have replied to user \textbf{I}'s tweet. The weights on the edges corresponds to the number of times user \textbf{I} and responder user interacted with each other}. Based on our dataset, we are only able to create one-hop network (ego-network) comprising of initiator of the tweet and its responders. \fixme{we can remove the Figure and text for this Figure if we need space. Please dO not be angry as you spend a lot of time on this Figure :)}
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=8cm,height=8cm,trim = {6cm 6cm 8cm 7cm}, clip, keepaspectratio]{Figures/Presentation2.pdf}
    \caption{Undirected Weighted Ego-Network of a Twitter User }\label{fig:ego_network}
\end{figure}

\end{enumerate}

It is important to note that the network formed between the initiator of the tweets and their corresponding responders naturally calls for a technique that can exploit network features as well. Thus, in order to capture the network properties, we employ Graph Neural Network (GNN) based approach for identifying possible \textit{rumor spreaders}.
To be specific, we explore Graph Convolutional Network (GCN), a particular
type of GNN for our analysis.
In contrast to the baseline approaches: SVM, RF, and LSTM, the GCN approach
exhibit better performance and is able to achieve a value of 0.864 for F1-Score and 0.720 for AUC-ROC Score. %\PS{Contribution and near ground truth?}
%\fixme{Let us discuss can we put a line about contribution somewhere? -- The contribution of this work is bla bla or 
To the best of our knowledge, this is the first work that has explored the \textbf{PHEME} dataset to identify possible \textit{rumor spreaders} using a weak supervised approach.

%\fixme{Following are not contributions. Contribution is in terms of framework -- IR + GCN + bla bla for misinformation spreaders.}
%\shakshi{The main contributions of this paper are as follows -

    % Due to lack of availability of the labeled rumor spreader dataset, we first use information retrieval techniques to transform the publicly available PHEME rumor dataset into rumor spreaders' dataset. Then, we apply weak supervised learning approach to annotate the ground truth of rumor spreaders. We apply supervised machine learning approaches to rumor spreaders dataset in order to validate the effectiveness of the transformation approach.     We show that GCN is a natural fit for our problem due to the inherent network structure of the rumor spreaders' dataset.

The rest of the paper is organized as follows.
Section \ref{sec:related} covers related work. Section \ref{sec:ds} covers dataset description and methodology used for identifying possible \textit{rumor spreaders}. Section \ref{sec:Evl} discusses experiments and their results, and Section \ref{sec:concl} concludes with some future directions.


\begin{comment}
\shakshi{\st{This paper deals with detecting suspicious users
on Twitter platform.
The users who often posts rumored tweets are likely to be the suspects.
Rumors are those when sender is un-aware about the information background at the time of posting, i.e. whether it is true or false.}

Twitter is a social network where each user can connect to another user using 3 mechanisms. First, following the another user, second, liking the tweet of other user, third, replying to the tweet of another user. Each user (either reply or posted the tweet) in the network is equally likely to be detected as suspicious or not suspicious user.
Thus, it is important to explore this type of network in our problem. Our main focus is on two types of users, reply users and the initiator users (who posts the original tweet) to detect suspicious users. Though, other features such as number of followers, tweets etc are also used in order to solve the problem.
To construct a network, nodes represents the users and edges are the connections between them such that if user 'A' who posts the tweet gets a reply from another user 'B' or vice-versa, then there would be an edge between the two. The weights on the edges represents the number of times users replied to each other. In order to preserve its network structure, we are utilizing GNN approach.
However, we have evaluated other traditional machine learning approaches as a baseline to prove that GNN is the best fit for our problem.
Our work is based on \textbf{PHEME} dataset which is publicly available on the Internet.
.}
\end{comment}






\begin{comment}
Based on the user intentions, spreading false information on social media can be broadly classified into two types - deliberately and mistakenly. By deliberately, it means that spreading the wrong information to the masses, just to create panic in the society or to gain some benefits (such as to change the stock market prices, to harm the reputation of the popular brands or to create instability in the country and many more), that leads to impact a state, a country, or even the world. The 2016 Campaign Elections is one of the great examples of spreading wrong information deliberately. This type of information is termed as \textbf{Disinformation}. By mistakenly, it means that spreading false or inaccurate information not to create any serious harm to the society. By inaccurate, it means that at the time of spreading the false information, either the sender is un-aware of the full facts or sender did not verify the source (origin) of the information.

%\st{this is how i strikeout }%
This type of information is termed as \textbf{Misinformation} \cite{karlova2013social}.
%\fixme{- ebla vbala bal} \shakshi{@Rajesh.. aactually what i wrote is correct. }%

Misinformation can be further classified into two types, Fake news and Rumor. 
\shakshi{@Rajesh Sir: Do i need to mention types of disinformation as well just like i did for misinformation? (Note: - I am working only on misinformation here.)}



According to \cite{zubiaga2018detection}, a general architecture for Rumor contains four sequential components - 

1. Rumor Detection - Having the posts (published by users on social media) as input to the model,  each post is labeled as either rumor or non-rumor to be used for identifying the rumor.

2. Rumor Tracking - After identifying the rumor, filter those posts that are related to particular rumor which eliminates irrelevant posts.

3. Stance Classification - Once the related posts are retrieved, each post is then labeled as supporting (the rumor), denying (the rumor), questioning (asking questions about the rumor) or commenting (about the rumor).

4. Veracity Classification - Having stance step as input or the rumor tracking step as input to the model, the truth value (veracity) of the rumor is predicted. The veracity of the rumor can be true, false or unproven. It could use URLs or other fact checking websites to collect information about the same. 

However, one or two components are explored in literature either in sequence or predicted simultaneously.



\subsection{Motivation}
There are two reasons for choosing this as a problem statement, first, detection of rumor in OSM platforms is a challenging task that requires immediate attention due to the fact that it is impossible for a common man to filter out which news is the rumor. %Though, we can detect the rumors and verified them in later stages either as true, false or unproven using various fact checking websites, such as politifact.com and many more. However, by the time rumor gets verified, the users already started to believe that rumor. Therefore, it is very crucial to detect rumor in a timely manner to avoid further spreading in the social network;
Second, mostly there are works in literature related to detection of rumor or determining its truth value etc. \shakshi{However, identifying suspicious user is more important than identifying rumored tweet in order to be more aware about those users who seems to be suspicious or more prone to publishing rumors on social websites. To the best of our knowledge, identifying suspicious users by utilizing reply networks is the first work.} %We are utilizing the user's reply network along with other features to detect suspicious users.


\subsection{Goal}
\shakshi{Our goal is to classify particular user is suspicious or not (a binary-classification problem) using supervised machine learning algorithms.}

%At a broad level, PHEME data set performing data pre-processing, machine learning algorithms are used to classify the final problem. A detailed explanation is in the Proposed Methodology section. 

\shakshi{The main contribution of our work is two-fold -}

\begin{enumerate}
    \item  Detection of suspicious users after performing data pre-processing steps and applying machine learning algorithms.
    \item Show that GNNs are more suitable for graph structured data.
\end{enumerate}

To conclude the paper, we have shown few of the possible future directions to extend our work.


\end{comment}

%1. Detect suspicious users by applying data pre-processing steps and machine learning algorithms.

%2. Show that GNNs are more suitable for our data or any type of data that can be modeled as a network or graph.






\begin{comment}


%\shakshi{@Rajesh: See what I ahev written -- new changed text}
What are OSM platforms (such as Twitter, Facebook), a social network or a news  media? \cite{kwak2010twitter}. These platforms initially developed for connecting peoples globally. %\shakshi{Need to look for a citation}
They have made the world smaller in a sense that everybody is reachable to any another person in the world. One of the concepts in graph theory - Six Degrees of Separation, states that it would take only six people (hops) to socially connect with another person in the world. However, this number seems to be changed by now. According to \cite{newyork}, based on Facebook data, (consisting of 721 millions of users of Facebook at the time of conducting this experiment), they found that on an average, any two persons are connected to each other with a 4.74 distance away, that is, it would only take four persons (hops) in between to connect with another person in the world. 

These platforms also evolved as a medium to spread false information to a large audience in a short period of time. This can cause panic, fear and financial loss to the society. Moreover, according to \cite{mitnews}, false information propagates six times faster than the true news in a social network. Thus, it is important to control them before it spreads to the masses.
\end{comment}

\begin{comment}
Along with strengthening the connectivity,
OSM platforms are having greater impact on everyone's lives on a regular basis.

Due to its increasing popularity among people, these platforms also evolved as a medium to spread false information to a large audience in a short period of time. This can cause panic, fear and financial loss to the society. Moreover, according to \cite{mitnews}, false information propagates six times faster than the true news in a social network. Thus, it is important to control them before it spreads to the masses.
\end{comment}

==> Shakshi-Rumor_Spreaders-IJCNN(15 jan 21)/related.tex <==
\section{Related work}\label{sec:related}
%\fixme{Rajesh@Shakshi: I will take care of this section.}
%In most of the previous studies, the social network problem has been formulated as a graph.

Researchers have proposed %\sout{various} \shakshi{numerous}
numerous techniques for identifying suspicious or fake user profiles across various OSM platforms such as Facebook \cite{gupta2017towards}, Twitter \cite{benevenuto2010detecting, wang2018sybilblind}, Tuenti  \cite{cao2012aiding}, to name a few. In this section, we discuss past studies across two dimensions. First, we %\sout{discuss work} \shakshi{talk about works} \sout{related} \shakshi{corresponding} 
discuss work related
to the identification of fake or suspicious users. Next, we %discuss works \sout{related} \shakshi{corresponding} 
present works about %to 
the detection of rumors. Our work lies at the intersection of these two types of works. %which this work lies.

\subsection{Suspicious Profile Detection}

Identification of suspicious (or fake) profiles on Twitter, a representative of OSM %\sout{such as}\shakshi{in particular} Twitter 
was initially %\sout{explored} \shakshi{analyzed} 
analyzed using apparent features %\sout{such as} \shakshi{for instance,}
such as the \textit{number of  followers} and the \textit{number of followings} \cite{benevenuto2010detecting}, \textit{user-profile-name, screen-name,  and  email  parameters} \cite{thomas2013trafficking} 
%\sout{on Twitter}. \sout{In addition} \shakshi{Moreover}, researchers analyzed the activity patterns of social media users such as the frequency of posting messages (or posts) on Facebook \cite{gupta2017towards} and Twitter \cite{gurajala2015fake}. \sout{Some other} \shakshi{Few other} works have also looked beyond individual users and considered social graph \cite{cao2012aiding, boshmaf2015method, wang2018sybilblind} and topological anomalies \cite{fire2012strangers}. %\fixme{Rajesh@Shakshi: please check --  Our work is different from these global approaches as they assumed the whole bird-eye view of the network compared to ours where we only are aware of ego-networks} \shakshi{ These papers are using global features apart from local features such as community, hubs and authorities, random walk.}. 
Our work is different from these global approaches as they assumed the whole bird-eye view of the network. %\sout{compared} \shakshi{in contrast}
In contrast, we are only aware of the ego-networks. %\sout{Some other}\shakshi{Further}
Some other works have focused on identifying suspicious followers by using multi-modal information \cite{jiang2014detecting}, which is out of the scope of this work.

%\subsubsection{MObile phone:}
It is a well-observed fact that mobile phones have been playing a %\sout{major}\shakshi{vital}
vital role in the popularity of OSM platforms. %\sout{However} \shakshi{Nonetheless}
Nonetheless, it has %\sout{also}
facilitated the rise of fake profiles %\shakshi{as well}
as well \cite{salehan2013social}. %\sout{Thus}  \shakshi{Therefore},
Therefore, mobile phones too have
%\shakshi{too} have \sout{also} 
been used as a medium in tracking fake profiles. %\sout{For example} \shakshi{For instance}
For instance, in \cite{perez2013dynamic}, the authors observed the daily behavior of users using mobile phone activity for detecting fake profiles. %\shakshi{Besides,} 
Besides researchers have %\sout{also}
also used camera-based sensors in detecting fake profiles within or across multi social networks \cite{bertini2015profile}.



\medskip

\subsection{Rumor Detection}

%\shakshi{Based on our assumption, }
%\shakshi{We assume that users who are often involved in disseminating rumors are more likely to be suspicious in comparison to users whose involvement in spreading rumor is less}. 
We assume that users who are often involved in disseminating rumors are more likely to be \textit{rumor spreaders} in comparison to users whose involvement in spreading rumor is less. Our approach for %\sout{detecting} \shakshi{identifying}
identifying the possible \textit{rumor spreaders} %\sout{use}\shakshi{leverage}
exploits (rumor and non-rumor) tweets %\sout{text} 
along with other features present in the dataset. %\sout{Thus}\shakshi{Therefore}
Therefore, we %\sout{also}\shakshi{further} 
further present related literature with respect to rumor detection.

%Rumor detection has attracted a lot of attention in the past few years due to advancements in the field of artificial intelligence techniques. Apart from AI based approaches, the past works include proposal of

%\sout{Compared} \shakshi{As opposed}
Initially starting with the theoretical framework for rumor spreading \cite{chierichetti2011rumor}, and later identification of rumors' temporal, structural, and linguistic features \cite{kwon2013prominent}, the topic related to rumor detection has attracted %\sout{a lot of}\shakshi{considerable} 
considerable attention in recent years, especially because of advancement in the field of artificial intelligence techniques. For example, in \cite{akhtar2018no}, %\sout{different}\shakshi{distinct}
various flavors of LSTM architecture are explored and in \cite{islam2019rumorsleuth}, a multi-task deep learning model is presented for rumor detection. In addition, %\sout{various other} \shakshi{several}
several techniques such as the use of particle swarm optimization  \cite{kumar2019rumour}, multi-modal approach by exploiting textual as well as visual features from the data \cite{singhal2019spotfake, wang2018eann}, have %\sout{also} 
also been %\sout{explored}\shakshi{examined} 
examined in the literature.

%In \cite{akhtar2018no}, author focused on the two tasks, stance classification and veracity of the rumor. Different flavors of LSTM architecture are explored on the SemEval-2017 dataset. 

%\sout{Some of the} \shakshi{Few}
Few approaches in rumor detection have also explored graph-based methodologies. %\sout{Such as}\shakshi{Specifically,}
Specifically, in \cite{rosenfeld2020kernel}, the authors constructed a Twitter follower graph and exploited diffusion patterns of
(mis) information for rumor detection. %\sout{Some of the}\shakshi{Further}
Some of the papers \cite{bian2020rumor, wei2019modeling, huang2019deep} have %\sout{also used} \shakshi{employed} 
employed Graph Convolutional Network (GCN) based approaches for detecting rumors.  
%\fixme{Rajesh@Shakshi -- please check -- However, compared to these works, our work is different that we are studying rumour text to understand suspicious users.}  \shakshi{Yes sir, this statement is true.}
%\sout{However, compared to} \shakshi{Unlike} 
Unlike these works, %\sout{our work is different as} we are studying 
we study the rumors to %\sout{detect}\shakshi{identify}
identify possible \textit{rumor spreaders}.

%\st{There have been some other works which have explored the user profiles as an important aspect in detecting rumor propagation either by analysing the profile of the user \cite{shu2019role}, identifying the source of the rumor \cite{devi2020veracity}, or based on the genuineness score for the users in the social network, which are spreading the rumors \cite{rath2017retweet}}
%\shakshi{Moreover, }
User profiles have %\sout{also} been \sout{explored} \shakshi{analyzed} 
been analysed as an important aspect in detecting rumor propagation. Analysis of the user profile \cite{shu2019role}, identification of source of the rumor \cite{devi2020veracity}, genuineness score %\sout{for}\shakshi{of}
of the users in the social network which are spreading the rumors \cite{rath2017retweet} have been %\sout{used}\shakshi{utilized}
utilized in the past works. 
Our work lies at the boundary of these works as our aim is to %\sout{detect} \shakshi{identify}
identify possible \textit{rumor spreaders} by %\sout{detecting} \shakshi{using}
using not only %\sout{using} 
the textual data that is being spread by these \textit{rumor spreaders} but also exploring their ego-networks. To accomplish this objective, we used GCN approach which has been mainly used in the past for %\sout{detecting}\shakshi{identifying}
identifying rumors and not for %\sout{detecting} \shakshi{identifying}
identifying possible \textit{rumor spreaders}. % in the past works.


\begin{comment}
%Most of the works on rumour detection have been based on Twitter data. For example, in \cite{rath2017retweet}, authors formulated the rumor problem as finding user is likely to spread rumor by utilizing the believability concept. The believability scores calculated are then assigned to the users in retweet network. 
%Detecting rumor at an early stage helps in stopping its spread. In \cite{parab2019twitter}, author has detected rumor in the first hour of publishing the post on Twitter by utilizing temporal characteristics of tweets.
 
%Researchers have also exploit the role of user profiles for fake news detection \cite{shu2019role}.  as well as  identifying source of the rumour \cite{devi2020veracity}.

%In \cite{monti2019fake}, author detected fake news at an early stage by utilizing GCN model. 
%In \cite{shu2019role}, to detect the same, author analyzed the role of user profiles.
%In \cite{devi2020veracity}, author focused on identifying the veracity of the rumor as well as finding the source of the rumor. This has been performed on one of the incidents, ‘Sydneyseige’ from PHEME dataset.


%In \cite{rosenfeld2020kernel}, author determined the veracity of rumor using diffusion pattern alone. They have constructed a Twitter follower graph with the help of Weisfeiler-Lehman graph kernel.






%In \cite{ma2019detect}, proposed a novel Generative-Adversarial Network (GAN) model to detect rumor considering the effect of information campaigns on rumor.


%\cite{jiang2014detecting}
 % Detecting suspicious following behavior in multimillion-node social networks: (a) synchro-nized behavior: the zombie followers have extremely similar following behavior pattern, because, say, they are generated by a script; and (b) abnormal behavior: their behavior pattern is very diﬀerent from the majority.
  
  
  %\cite{rostampour2014method}
  %Method for detecting suspicious individuals in a friend list
  %\cite{wang2018sybilblind}
  %Detecting fake users in online social networks without manual labels
  
  
 % \cite{perez2013dynamic}
  %A dynamic approach to detecting suspicious profiles on social platforms: mobile social networking site user.on based on their daily behaviour.





%===============================

%In \cite{bodaghi2018novel}, author studied the psycho-sociological factors that can influence the mind of the user to spread the rumor (anti-rumor). He believes that these factors lead to better understanding of the spread of the rumor in social networks. 




%\subsection{Misinformation Diffusion}
%In \cite{monti2019fake}, author detected fake news at an early stage by utilizing GCN model. 
%In \cite{shu2019role}, to detect the same, author analyzed the role of user profiles.

%In \cite{akhtar2018no}, author focused on the two tasks, stance classification and veracity of the rumor. Different flavors of LSTM architecture are explored on the SemEval-2017 dataset. 
%In \cite{rosenfeld2020kernel}, author determined the veracity of rumor using diffusion pattern alone. They have constructed a Twitter follower graph with the help of Weisfeiler-Lehman graph kernel. 

%In \cite{kumar2019rumour}, author used a particle swarm optimization technique in identifying the veracity of the rumor.
%In \cite{islam2019rumorsleuth}, proposed a multi-task deep learning model, RumorSleuth to jointly detect stance and veracity of the rumor.

 

%In \cite{yuan2019jointly}, author proposed a novel model for rumor, global-local attention network that captures the local semantic and global structural information.

%There is a lack of enough labeled data in rumor. In [Wen, Sooji Han] \cite{han2019neural}, author tried to overcome the same. The unlabeled rumor data is  augmented with the help of a neural language  model. Their augmented data set achieves good results.

%\subsection{multi modal}
% textual as well as visual features from the data
%In \cite{singhal2019spotfake}, author claims that the multi-modal fake news detection problem is considered to be the secondary task in literature. This tends to decrease their performance. So, their goal is to take this as a primary task. They used BERT  model for text and pre-trained VGG-19 model for images on Twitter and Sina Weibo data sets.

%In \cite{wang2018eann}, author identified the fake news on new events. Their approach involves multi-modal extractor which extracts the textual as well as visual features from the data. Fake news detector and adversarial neural networks are explored here.

%In \cite{tam2019anomaly,chen2018unsupervised}, modeled the rumor problem as an anomaly detection problem. Former utilized a multi-modal approach to identify the anomaly. Latter, exploited the unsupervised learning approach. Their model is a combination of RNN and Autoencoder deep learning techniques on the Sina Weibo data set.

%\subsection{rumour problem as a network}
%In \cite{chierichetti2011rumor}, author studied the rumor problem as a typical preferential attachment model. However, preferential attachment model is not well suited for complex networks.

%In \cite{kwon2013prominent}, author identified the temporal, structural and linguistic features of rumor by considering it as a diffusion network problem.



 


%In \cite{ma2019detect}, proposed a novel Generative-Adversarial Network (GAN) model to detect rumor considering the effect of information campaigns on rumor.


%\subsection{Tweet}
%In \cite{rath2017retweet}, author formulated the rumor problem as finding user is likely to spread rumor by utilizing the believability concept. The believability scores calculated are then assigned to the users in retweet network. 
%Detecting rumor at an early stage helps in stopping its spread. In \cite{parab2019twitter}, author has detected rumor in the first hour of publishing the post on Twitter by utilizing temporal characteristics of tweets.



%Detection of rumor in a health domain is essential to the society.
%In \cite{sicilia2018twitter}, author introduced various novel features for performing rumor detection in the health domain sector utilizing various machine learning approaches. 

%Detecting rumor at an early stage helps in stopping its spread. In \cite{parab2019twitter}, author has detected rumor in the first hour of publishing the post on Twitter by utilizing temporal characteristics of tweets.
 
%In \cite{gupta2014tweetcred}, author developed a browser plugin called “TweetCred” that assigns a credibility score with respect to tweets in a user’s timeline by applying various machine learning approaches.

%In \cite{singh2020predicting}, author predicted the popularity of rumors on Twitter data sets using various machine learning approaches.




\subsection{GCN}
In \cite{bian2020rumor}, their work is based on the novel Bi-directional GCN that focuses on the network structure of rumors.
In \cite{wei2019modeling}, author performed stance and veracity simultaneously using both GCN and Recurrent Neural Network (RNN) wherein nodes represent the tweets and the edges represent the replies of tweets.

In \cite{huang2019deep}, author used GCN to obtain the user behavior to better predict the rumor. \fixme{our work is different that we are studying rumor text to understand possible rumor spreaders.} 



\subsection{Competitions related to rumor have been carried out on the web like in} \cite{janchevski2019andrejjan}, author performed the task as a part of SemEval task – 2019. Their focus is on finding the veracity of the rumor using traditional, ensemble-based and neural network classifiers. 
Similarly another task, a RumorEval shared task, focused on two tasks – stance and veracity prediction. Submission results are shown in \cite{gorrell2019semeval}.

In \cite{wang2019modeling}, author modeled the rumor propagation problem as a negative energy model to mitigate the chance of spreading rumor from interconnected social networks.


%For  fast  detection  of  spam  accounts,  a  simple  profile-pattern detection  without detailed  “Tweet”  analysis  has  been proposed \cite{thomas2013trafficking}.    For  example,  Benevenuto  et  al.  \cite{benevenuto2010detecting} used  profile information  such  as  “number  of  followers  and  number  of followings” to identify fake profiles.  Thomas et al. \cite{thomas2013trafficking} used a multi-variable  pattern-recognition  approach  based  on  user-profile-name,  screen-name,  and  email  parameters.  

 %\cite{gurajala2015fake}
  %Fake Twitter accounts: profile characteristics obtained using an activity-based pattern detection approach
  
  %\fixme{Following is the copy paste from %\cite{gurajala2015fake}}
  %For  fast  detection  of  spam  accounts,  a  simple  profile-pattern detection  without detailed  “Tweet”  analysis  has  been proposed \cite{thomas2013trafficking}.    For  example,  Benevenuto  et  al.  \cite{benevenuto2010detecting} used  profile information  such  as  “number  of  followers  and  number  of followings” to identify fake profiles.  Thomas et al. \cite{thomas2013trafficking} used a multi-variable  pattern-recognition  approach  based  on  user-profile-name,  screen-name,  and  email  parameters. 
  
  %\cite{gupta2017towards} Towards detecting fake user accounts in Facebook
  

  \cite{bertini2015profile}Profile resolution across multilayer networks through smartphone camera fingerprint
\cite{bertini2015smartphone} Smartphone verification and user profiles linking across social networks by camera fingerprinting
---
Mobile phone plays an important role .. so by tracking t \cite{perez2013dynamic}


\cite{cao2012aiding}
  Aiding the detection of fake accounts in large scale social online services: It relies on social graph
properties to rank users according to their perceived likelihood of being fake (Sybils)
, later graph related features were also used \cite{boshmaf2015method} : random walk

 \cite{fire2012strangers}
  Strangers intrusion detection-detecting spammers and fake profiles in social networks based on topology anomalies
\cite{boshmaf2015method}
 Method and system for predicting victim users and detecting fake user accounts in online social networks
   a 
graph-based detector for detecting fake users by computing
through the power iteration method a probability of a random
walk to
\end{comment}

==> background.tex <==
\section{Graph Convolutional Network}\label{sec:gcn}
\medskip

\sout{GNN is a new and popular branch of machine learning that operates on non-Euclidean data. Data that inherently forms a network is a good fit for GNN. For instance, citation network, social network,  protein-protein interaction network, to name a few. Unlike network embedding approaches (such as DeepWalk \cite{perozzi2014deepwalk}, node2vec \cite{grover2016node2vec}), GNN captures the graph properties. In particular node attributes and can be generalized to unseen nodes (graphs) as well. There exist multiple variants of GNN such as Graph Convolution, Graph Autoencoder, Graph Recurrent Neural Network.
    
Graph Convolution is a %\sout{specific kind} \shakshi{particular type} 
particular type of GNN and %\sout{the Graph Convolution} \shakshi{its} 
its framework is inspired from Convolutional Neural Network \cite{krizhevsky2012imagenet}. Based on kernel selection, Graph Convolution can be bifurcated into two classes, spectral based and spatial based. In spectral based kernel selection, inputs are transformed into the spectral domain with the help of eigenvalue decomposition wherein the kernel, and the transformed input gets convolved. Furthermore, the transformed inputs bring back to the original domain in order to be used by next layer in the network. In comparison, spatial based kernel selection aggregates the information of neighboring nodes by itself in order to maintain the topology of the network. The aggregated information fetched from the previous layer is then passed to the following layer in network \cite{wu2020comprehensive, hamilton2017representation}. This idea of message passing is inspired from Recurrent Neural Network (RNN).
    
    
    Graph Convolutional Network (GCN) \cite{kipf2016semi} is a spectral based two-layer network designed for the semi-supervised node classification task. The inputs to GCN are features matrix of dimension \textit{$N$X$F$} and symmetric adjacency matrix of dimension \textit{$N$X$N$}, where \textit{N} is the number of nodes in the graph and \textit{F} is the number of features.
    
    Following is the propagation rule for every layer in the network. This rule is inspired from first-order approximation of localized spectral filters on graphs \cite{kipf2016semi}.
    \begin{equation}
    \boldsymbol{H^{(l+1)} = \sigma (\Tilde{D}^{-0.5}   \: \Tilde{A}\:  \Tilde{D}^{-0.5}\:  H^{(l)} \: W^{(l)})},
    \end{equation}
   
    %\shakshi{Need to write dimension of hidden layer, change mathematical notations.}
    where, \textit{H\textsuperscript{(l+1)}} 
    represents the current hidden layer, \textit{\(\sigma\)}
    is the non-linear activation function, \textit{\(\Tilde{D}\)\textsuperscript{-0.5}}  is the normalized degree matrix, 
    \textit{\(\Tilde{A}\)}
    represents symmetric adjacency matrix with self-connections, \textit{W\textsuperscript{(l)}} is the learnable weight matrix parameter of previous hidden layer.
  
    At layer \textit{l = 0},
    \begin{equation*}
        \boldsymbol{H^{(0)} \: = X}   
    \end{equation*}
    where \textit{X} represents the nodes' features matrix %\shakshi{of dimension \textit{$N$X$F$}}.
    of dimension \textit{$N$X$F$}.
    The last layer is used for classification. Number of nodes in the last layer depend on number of classes. After building the model, the weights are trained using stochastic gradient descent algorithm  until either a loss function is minimized to  a certain defined level or model completed a specified number of iterations (or epochs).
    }
